Surrogate Scoring Rules

Strictly proper scoring rules (SPSR) are incentive compatible for eliciting information about random variables from strategic agents when the principal can reward agents after the realization of the random variables. They also quantify the quality of elicited information, with more accurate predictions receiving higher scores in expectation. In this paper, we extend such scoring rules to settings where a principal elicits private probabilistic beliefs but only has access to agents' reports. We name our solution \emph{Surrogate Scoring Rules} (SSR). SSR build on a bias correction step and an error rate estimation procedure for a reference answer defined using agents' reports. We show that, with a single bit of information about the prior distribution of the random variables, SSR in a multi-task setting recover SPSR in expectation, as if having access to the ground truth. Therefore, a salient feature of SSR is that they quantify the quality of information despite the lack of ground truth, just as SPSR do for the setting \emph{with} ground truth. As a by-product, SSR induce \emph{dominant truthfulness} in reporting. Our method is verified both theoretically and empirically using data collected from real human forecasters.

==> discussion.tex <==
%\subsection*{Additional proof to the proof of Lemma \ref{lemma:est}}\label{sec:het}
%
%
%  In this section we present the additional proof to the one of Lemma \ref{lemma:est} as detailed in \cite{LC17}; particularly we would like to show the estimation error results extend to the case with heterogeneous agents and asymmetric strategies. The primary change lies in the fact that the  estimation of $p_{1,z},p_{0,z}$ is different. The reason is as follows. Again we can formulate a system of quadratic equations as in Mechanism \ref{p_estimate}. But note if we assign one label to two different workers, due to the asymmetric error rate, the LHS of Eqn. (I) is not precise-- drawing a worker without replacement leads to a different labeling accuracy, and will complicate the solution for the system of equations. 
%
%One very natural solution is when we re-assign a task, we randomly select a worker from the entire candidate set (selection with replacement), the quadratic equations for estimating $p_{1,z},p_{0,z}$ become identical with the ones in Mechanism \ref{p_estimate}. In order to do so,  we need to assume that when a worker is assigned the same task twice, the two copies are generated in an IID fashion -- this assumption is backed up by the "crowd within" effects \cite{VulPashler2008}. Also due to the difference in workers' expertise level, simply separating the workers into two groups and use one group for learning the matching probability will not work. \rev{Since now each worker may be assigned two tasks, we made an additional requirement that the uninformative strategies stay the same for both assigned tasks.} Similarly when $K$ is large enough, truth telling is a BNE $\forall i$. The reason for above claim is very similar to the one for our main theorem.
%
%W next show a direct estimation -- without replacement -- will not affect our results by too much: denoting by $p_1$ the accuracy of first drawn sample (for checking the matching) when $y=1$ (we can similarly argue for $y=0$). Then we have $\mathbb E[p_1] = p_{1,z}$. And the average accuracy of the second drawn sample $p_2$ (conditional on $p_1$) is given by  $\frac{p_{1,z} (N-1) - p_1}{N-2}$. Further the matching probability satisfies the following:
%\begin{align*}
%\mathbb E[p_1 \cdot p_2 ] &= \mathbb E\biggl [ \mathbb E[p_1 \cdot p_2|p_1] \biggr]=\mathbb E\biggl [ p_1 \cdot \frac{p_{1,z} (N-1) - p_1}{N-2} \biggr] \\
%&=\mathbb E[p_1] \cdot \frac{p_{1,z} (N-1)}{N-2} - \frac{\mathbb E[p^2_1]}{N-2} = \frac{N-1}{N-2} p^2_{1,z}  -  \frac{\mathbb E[p^2_1]}{N-2}
%\end{align*}
%Note both $p_{1,z}$ and $\mathbb E[p^2_1]$ are no more than 1. Then 
%\begin{align*}
%|\frac{N-1}{N-2} p_{1,z}  -  \frac{\mathbb E[p^2_1]}{N-2} -p^2_{1,z} | \leq \frac{|p^2_{1,z}|}{N-2} + \frac{\mathbb E[p^2_1]}{N-2} \leq \frac{2}{N-2}.
%\end{align*}
%That the estimated quantity is bounded away from the true parameter by at most $O(1/N)$. Then the error analysis in \cite{LC17} tells us that when $N$ is large enough, our mechanism will remain properness. 
%
%
%
%In fact that the above analysis show we can afford a $O(\log N)$ discrepancy as $O(\frac{\log N}{N})$ would still be diminishing with an increasing $N$. That means when select the two reference answers, the candidate population can differ by $O(\log N)$ number of agents, instead of only 1. 
\section{Discussions}\label{sec:conclude}


Below we make a couple of remarks, discuss possible caveats and their possible fix. %We further extend SSR to the peer prediction setting where the noisy ground truth can only be inferred via collecting reports from other reference agents. This returns us a \emph{dominant truth serum} (DTS). Both. % which achieves truthful elicitation in dominant strategy.


%\paragraph{Recovering the ground truth}

%Though being a fundamental step, truthful elicitation is also often not the ultimate goal, as the mechanism designer may want to infer the ground truth answer in the end. As a by-product, our framework for inferring the error rates from agents would allow us to do so. The reasoning is as follows: first ask each agent $j \neq i$ to report a label. If the ground truth label is 0, the posterior distribution of agents' reports being 1 will converge to $e_{0,z}$ with high probability; while on the other hand, if the ground truth is 1, this posterior distribution converges to $1-e_{1,z}$. When $e_{0,z} \neq 1-e_{1,z}$ (reference answer being informative), we will know the ground truth label with high probability via posterior distribution testing. 

%\paragraph{Unbiased estimator of the true score} 


%Our paper proposes a novel and robust way for quantifying the quality of information when there is no ground truth verification, using peer evaluation, as well as an estimation procedure for learning the bias in peer evaluation. This may find applications in a sequential elicitation setting, where such scores can provide informative feedbacks to contributed information before the outcome reveals.
%In our work we do require the mechanism designer to know the priors (of the ground truth, not agents' private information). Such statistical information can be estimated from historical information (of similar events), or from cheap surveys. Also we would like to point out that our solution is robust to small perturbation of priors, as evidenced by the finite sample error analysis. 




\subsection{Weak dominance v.s. strong dominance}

We have shown when we cannot learn an informative enough reference report from the rest of the agents, there is very little we can do regarding that. With this note, our deterministic payment strategy is only weakly dominant. We argue that if agents' reports can be modeled as being from certain distributions, the weak dominance case happens rarely. 


Denote by $X_i = \tilde{e}_{1,i}+\tilde{e}_{0,i}$, the weakly dominant case happens only when $\sum_{j \neq i} X_j = 1$. Potentially there are infinitely many strategies that lead to this state. However, suppose agents' reporting strategies are drawn from a distribution defined over a continuous space (mixed strategy space), then we can easily argue that $\{\omega: \sum_{j \neq i} X_j(\omega) = 1\}$ (via taking $\sum_{j \neq i} X_j$ as a random variable)  is a zero measure event. 

Also we would like to point out that, as long as each agent believes that this uninformative state happens with probability $<1$, DTS induces strong dominant strategy in truthful reporting, as a non-trivial mix between weak and strong dominance returns strong dominance.

Also, as a matter of fact, $\sum_{j \neq i} X_j = 1$ corresponds to the case that the reference signal is \emph{stochastically irrelevant} to the ground truth. Theoretically speaking, there is little one can do for eliciting private signals using such a reference signal, via a peer prediction method. In practice, one can use screening tasks to remove some workers to move away from this uninformative state.



\subsection{Effort exertion} 

So far our discussion focuses on eliciting truthful reports, our results extend to the scenario for eliciting high quality data. For instance, when workers can choose to exert costly effort (consider a binary effort level case, and denote the cost as $c$ for exerting efforts) to improve the quality of their answers, and once the reference signal is informative (either positively or negatively), we can scale up the scoring functions to cover the cost $c$, as similarly done in \citep{MRZ:2005}, to establish the dominance of reporting a high-effort signal. 


\subsection{Heterogeneous error rates across tasks}

In order to estimate error rates correctly, we needed to make the assumption that human workers have homogeneous error rates across multiple tasks. We now discuss the applicability of our method in light of the heterogeneity issue. Before starting, we would like to emphasize that in practice, for each set of experiments we can choose to group tasks according to their types (e.g., image labeling, solving puzzles, objects recognition), and run our mechanism over each group separately. For this setting, we can assume the homogeneity more comfortably. 

Nonetheless when it is not quite possible to group tasks together, suppose that each human agent's error rates are also task contingent in that for each possible task $x$ with $y \sim \mathcal P:=\{\mathcal P_0, \mathcal P_1\}$ we have $e_{0,i}(y), e_{1,i}(y)$. Redefine the error rate of the reference answer as follows:
\begin{align*}
e_{1,z} = \frac{\sum_{j \neq i} \mathbb E_{x,y|y=1} [e^r_{1,j}(x)]}{N-1},~
e_{0,z} = \frac{\sum_{j \neq i} \mathbb E_{x,y|y=0} [e^r_{0,j}(x)]}{N-1}.
\end{align*}
Again $e_{1,z} ,e_{0,z} $ captures the error rate of the reference answer. With knowing $e_{1,z}, e_{0,z} $, the dominant strategy argument in Theorem \ref{noise:learn} holds. 

So far so good. However it becomes less clear in how to estimate $e_{1,z}, e_{0,z} $. If we follow the idea in Section \ref{sec:bias:learn}, the first order equation holds as before
\[
\mathcal P_0 \frac{\sum_{j \neq i} \mathbb E_{x,y|y=0} [e^r_{0,j}(x)]}{N-1} + \mathcal P_1(1- \frac{\sum_{j \neq i} \mathbb E_{x,y|y=1} [e^r_{1,j}(x)]}{N-1}) = P_{1,-i}, 
\]
i.e., 
$
\mathcal P_0 e_{0,z} + \mathcal P_1(1-e_{1,z}) = P_{1,-i}.
$
However the higher order matching statistics appear to be very different. For example, the second order matching probability between two agents on label $1$ becomes 
\[
\mathcal P_0 \frac{\sum_{j \neq i} \mathbb E_{x,y|y=0} [(e^r_{0,j}(x))^2]}{N-1} + \mathcal P_1\frac{\sum_{j \neq i}\mathbb E_{x,y|y=1}[1-(e^r_{1,j}(x))^2]}{N-1} = P_{1,-i}, 
\]
Instead we would like a equation as a function of $$
\biggl (\frac{\sum_{j \neq i} \mathbb E_{x,y|y=0} [e^r_{0,j}(x)]}{N-1} \biggr)^2, \biggl(\frac{\sum_{j \neq i}\mathbb E_{x,y|y=1}[1-e^r_{1,j}(x)]}{N-1}\biggr)^2$$
in order to identify the true error rates on average. To get around of this issue, we can adopt the following approximation for $(e^r)^2_{0,j}(x)$ using Taylor expansion:
\[
(e^r_{0,j}(x))^2 \approx e^2_{0,z} +2e_{0,z}(e^r_{0,j}(x)-e_{0,z}) = 2e_{0,z} \cdot e^r_{0,j}(x) - e^2_{0,z}.
\]
Then we claim that
\begin{align*}
\frac{\sum_{j \neq i} \mathbb E_{x,y|y=0} [(e^r_{0,j}(x))^2]}{N-1} &\approx \frac{\sum_{j \neq i} \mathbb E_{x,y|y=0} [2e_{0,z} \cdot e^r_{0,j}(x) - e^2_{0,z}]}{N-1} \\
&= 2e_{0,z} \cdot e_{0,z} - e^2_{0,z} = e^2_{0,z}
\end{align*}
Similarly we have
\begin{align*}
\frac{\sum_{j \neq i}\mathbb E_{x,y|y=1}[1-(e^r_{1,j}(x))^2]}{N-1} \approx (1-e_{1,z})^2.
\end{align*}
From above, we see we are able to recover the matching equations defined in our earlier solution for task homogeneous cases; and it can be viewed as a linear approximation for this task contingent case. 


%\paragraph{Heterogeneous error rates}
%
%In order to estimate error rates correctly, we needed to make the assumption that agents have homogeneous error rates over multiple tasks. We now discuss the applicability of our method in light of the heterogeneity issue. First we would like to emphasize that in practice, for each set of experiments we can choose to group tasks according to their types (e.g., image labeling, solving puzzles, objects recognition), and run our mechanism over each group separately. For this setting, we can assume the homogeneity more comfortably. When it is not quite possible to group tasks together, suppose that each human agent's error rates are also task contingent in that for each possible task, we show our solution can be viewed as a linear approximation for this task contingent case. We have more details on this matter in the Appendix.

%\paragraph{Quality of information}

\subsection{A Machine Learning method}

To echo recent works on using machine learning techniques \cite{LC17} to learn a machine learning model to generate a reference answer, instead soliciting from other agents, we show this idea is also ready to be plugged into our SSR solution framework. Consider the current task that needs to be elicited and denote its feature vector as $\mathbf{x} \in \mathbb R^d$. Suppose we have learned (following the results in \cite{LC17}, such a classifier is learnable purely from agent's reported noisy data) a good classifier $\tilde{f}^*(\mathbf{x})$ for predicting its true outcome. Replace the reference answer $z$ with $\tilde{f}^*(\mathbf{x})$ and plug in its error rates. The rest of job is to reason about $e_{1,z},e_{0,z}$ (for $\tilde{f}^{*}(\mathbf{x})$). There are possibly many different ways to do so. %We sketch its possibility when there is again no ground truth label being available in Appendix.

Suppose that each task is associated with a corresponding feature vector. Consider the current task that needs to be elicited and denote its feature vector as $\mathbf{x} \in \mathbb R^d$. Suppose we have learned (following the results in \cite{LC17}, such a classifier is learnable purely from agent's reported noisy data) a good classifier $\tilde{f}^*(\mathbf{x})$ for predicting its true outcome. Our ML-aided SSR simply works in the following ways: replacing the reference answer $z$ with $\tilde{f}^*(\mathbf{x})$ and plug in its error rates. The rest of job is to reason about $e_{1,z},e_{0,z}$ (for $\tilde{f}^{*}(\mathbf{x})$). There are possibly many different ways of doing so. We demonstrate its possibility when there is again no ground truth label being available with the following simple estimation procedure:
\begin{itemize}
\item Assign $K$ tasks $\mathbf{x}_1, \mathbf{x}_2, ...,\mathbf{x}_K$ to three randomly drawn peers, denote them as $z^{\text{ref}}_{i}(\mathbf{x}_k), i=1,2,3, ~k=1,2,...,K$.
\item Estimate $\Pr[\tilde{f}^*(\mathbf{x}_i) = z^{\text{ref}}_1(\mathbf{x}_i) = 1] $ and $\Pr[\tilde{f}^*(\mathbf{x}_i)  = 1]$.
\item Estimate $\Pr[z^{\text{ref}}_1(\mathbf{x}_i) = 1|y=0]$ (follow Mechanism \ref{p_estimate}) using the three reference answers $z^{\text{ref}}_{i}(\mathbf{x}_k), i=1,2,3, ~k=1,2,...,K$.
\end{itemize}
Then note the following fact:
\begin{align*}
&\Pr[\tilde{f}^*(\mathbf{x}_i) = z^{\text{ref}}_1(\mathbf{x}_i) = 1]\\
 =& \mathcal P_0 \Pr[\tilde{f}^*(\mathbf{x}_i) = 1|y=0] \Pr[z^{\text{ref}}_1(\mathbf{x}_i) = 1|y=0] \\
+ &\mathcal P_1 \Pr[\tilde{f}^*(\mathbf{x}_i) = 1|y=1] \Pr[z^{\text{ref}}_1(\mathbf{x}_i) = 1|y=1]
\end{align*}
Together with 
\[\Pr[\tilde{f}^*(\mathbf{x}_i)  = 1] = \mathcal P_0 \Pr[\tilde{f}^*(\mathbf{x}_i) = 1|y=0]+ \mathcal P_1 \Pr[\tilde{f}^*(\mathbf{x}_i) = 1|y=1],\]
 we will be able to solve for $e_{1,z},e_{0,z}$ when we have a good estimates of $\Pr[\tilde{f}^*(\mathbf{x}_i) = z^{\text{ref}}_1(\mathbf{x}_i) = 1]$ and $\Pr[\tilde{f}^*(\mathbf{x}_i)  = 1] $, and that $\Pr[z^{\text{ref}}_1(\mathbf{x}_i) = 1|y=0] \neq \Pr[z^{\text{ref}}_1(\mathbf{x}_i) = 1|y=1]
$. With above argument, we see that we will be able to achieve dominant strategy scorings without even the need of reassigning all tasks.
%

